CloudSim 7G: An Integrated Toolkit for Modeling and Simulation of Future Generation Cloud Computing Environments

Cloud Computing has established itself as an efficient and cost-effective paradigm for the execution of web-based applications, and scientific workloads, that need elasticity and on-demand scalability capabilities. However, the evaluation of novel resource provisioning and management techniques is a major challenge due to the complexity of large-scale data centers. Therefore, Cloud simulators are an essential tool for academic and industrial researchers, to investigate the effectiveness of novel algorithms and mechanisms in large-scale scenarios. This paper proposes CloudSim 7G, the seventh generation of CloudSim, which features a re-engineered and generalized internal architecture to facilitate the integration of multiple CloudSim extensions within the same simulated environment. As part of the new design, we introduced a set of standardized interfaces to abstract common functionalities and carried out extensive refactoring and refinement of the codebase. The result is a substantial reduction in lines of code with no loss in functionality, significant improvements in run-time performance and memory efficiency (up to 25% less heap memory allocated), as well as increased flexibility, ease-of-use, and extensibility of the framework. These improvements benefit not only CloudSim developers but also researchers and practitioners using the framework for modeling and simulating next-generation Cloud Computing environments.

==> Makefile <==
MAIN=main
TEX_FILES = $(MAIN).tex
 
all: $(MAIN).pdf

%.pdf: %.tex $(shell find src/ -name '*.tex') $(wildcard *.bib)
	pdflatex $<
	bibtex $(<:.tex=)
	pdflatex $<
	pdflatex $<

clean:
	rm -f *~ *.bak *.aux *.out *.abs *.log *.bbl *.blg $(MAIN).pdf main-diff-*.pdf

PREF:=$(shell git rev-parse --show-prefix)

## Type `make main-diff-<commit-id>.pdf` to get a .pdf showing the differences
## between <commit-id> and HEAD.
## NOTE: due to a latexdiff bug (https://github.com/ftilmann/latexdiff/issues/5),
## diffs in tables are not always handled correctly, so we ignore them altogether.
define diff_templ
$(1)-diff-%.tex: /tmp/diff-%.dir $(1).tex $(filter-out $(1)-diff-%,$(wildcard *.tex *.bib)) main.pdf
	cd $$</$(PREF) && make; touch main.tex && make
	latexdiff --encoding=utf8 --config="PICTUREENV=(?:picture|DIFnomarkup|tabular)[\w\d*@]*" --exclude-safecmd=ref --disable-citation-markup --disable-citation-markup --flatten $$</$(PREF)$(1).tex $(1).tex > $$@
endef

$(foreach p,$(TEX_FILES:.tex=),$(eval $(call diff_templ,$(p))))

/tmp/diff-%.dir:
	git clone --reference $(shell git rev-parse --show-toplevel) \
	$(shell git remote -v | grep origin | grep fetch | sed -e 's#origin[[:blank:]]\+##; s/ (fetch)//') $@ \
	&& cd $@ \
	&& git checkout $(patsubst /tmp/diff-%.dir,%,$@)
	cp main.bib $@/$(PREF)


